Brick wall diagrams as a completely integrable system

We study the free energy of an integrable, planar, chiral and non-unitary four-dimensional Yukawa theory, the bi-fermion fishnet theory discovered by Pittelli and Preti. The typical Feynman-diagrams of this model are of regular "brick-wall"-type, replacing the regular square lattices of standard fishnet theory. We adapt A. B. Zamolodchikov's powerful classic computation of the thermodynamic free energy of fishnet graphs to the brick-wall case in a transparent fashion, and find the result in closed form. Finally, we briefly discuss two further candidate integrable models in three and six dimensions related to the brick wall model.

==> bibdatei <==
@article{Zamolodchikov:1980mb,%Zamolodchikov_1980
    author = "Zamolodchikov, A. B.",
    title = "{'FISHNET' DIAGRAMS AS A COMPLETELY INTEGRABLE SYSTEM}",
    doi = "10.1016/0370-2693(80)90547-X",
    journal = "Phys. Lett. B",
    volume = "97",
    pages = "63--66",
    year = "1980"
}

@article{Bazhanov:2016ajm,%Bazhanov_2016
    author = "Bazhanov, Vladimir V. and Kels, Andrew P. and Sergeev, Sergey M",
    title = "{Quasi-classical expansion of the star-triangle relation and integrable  systems on quad-graphs}",
    eprint = "1602.07076",
    archivePrefix = "arXiv",
    primaryClass = "math-ph",
    doi = "10.1088/1751-8113/49/46/464001",
    journal = "J. Phys. A",
    volume = "49",
    number = "46",
    pages = "464001",
    year = "2016"
}

@article{bousquetmelou1999inversion,%Bousquet_1999
      title={Inversion relations, reciprocity and polyominoes}, 
      author={M. Bousquet-Melou and A. J. Guttmann and W. P. Orrick and A. Rechnitzer},
      year={1999},
      eprint={math/9908123},
      archivePrefix={arXiv},
      primaryClass={math.CO}
}

@article{Bombardelli:2016scq,%Bombardelli_2016
    author = "Bombardelli, Diego",
    title = "{S-matrices and integrability}",
    eprint = "1606.02949",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1751-8113/49/32/323003",
    journal = "J. Phys. A",
    volume = "49",
    number = "32",
    pages = "323003",
    year = "2016"
}

@article{Zamolodchikov:1976uc,%Zamolodchikov_1977_ExactSMatrix
    author = "Zamolodchikov, A. B.",
    title = "{Exact s Matrix of Quantum Sine-Gordon Solitons}",
    reportNumber = "ITEP-148-1976",
    journal = "JETP Lett.",
    volume = "25",
    pages = "468",
    year = "1977"
}

@article{Pokrovsky_1982,
       author = {{Pokrovsky}, S.~V. and {Bashilov}, Yu. A.},
        title = "{Star-triangle relations in the exactly solvable statistical models}",
      journal = {Communications in Mathematical Physics},
         year = 1982,
        month = mar,
       volume = {84},
       number = {1},
        pages = {103-132},
          doi = {10.1007/BF01208374},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982CMaPh..84..103P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System},
      url = {\url{https://link.springer.com/article/10.1007/BF01208374}}
}

@article{StroganovInvRelLatticeModels,
	title = {A new calculation method for partition functions in some lattice models},
	journal = {Physics Letters A},
	volume = {74},
	number = {1},
	pages = {116-118},
	year = {1979},
	issn = {0375-9601},
	doi = {https://doi.org/10.1016/0375-9601(79)90601-7},
	url = {https://www.sciencedirect.com/science/article/pii/0375960179906017},
	author = {Yu.G. Stroganov}
}

@article{Shankar:1977cm,%ShankarWittenInvRel
    author = "Shankar, R. and Witten, Edward",
    title = "{The S Matrix of the Supersymmetric Nonlinear Sigma Model}",
    reportNumber = "HUTP-77/A076",
    doi = "10.1103/PhysRevD.17.2134",
    journal = "Phys. Rev. D",
    volume = "17",
    pages = "2134",
    year = "1978"
}

@article{Baxter:1982xp,%Baxter_1982_InvRel2DLattice
    author = "Baxter, R. J.",
    title = "{The inversion relation method for some two-dimensional exactly solved models in lattice statistics}",
    doi = "10.1007/BF01011621",
    journal = "J. Statist. Phys.",
    volume = "28",
    pages = "1--41",
    year = "1982"
}

@article{Baxter:1989ct,%Baxter_1989_Solving
    author = "Baxter, R. J.",
    title = "{Solving models in statistical mechanics}",
    journal = "Adv. Stud. Pure Math.",
    volume = "19",
    pages = "95",
    year = "1989"
}

@article{Baxter:2002qg,%Baxter_2003_InvRelPottsModel
    author = "Baxter, R. J.",
    title = "{The 'Inversion relation' method for obtaining the free energy of the chiral Potts model}",
    eprint = "cond-mat/0212075",
    archivePrefix = "arXiv",
    doi = "10.1016/S0378-4371(02)02024-1",
    journal = "Physica A",
    volume = "322",
    pages = "407--431",
    year = "2003"
}

@article{Beisert:2010jr,%IntegrabilityAdSCFTreview
    author = "Beisert, Niklas and others",
    title = "{Review of AdS/CFT Integrability: An Overview}",
    eprint = "1012.3982",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "AEI-2010-175, CERN-PH-TH-2010-306, HU-EP-10-87, HU-MATH-2010-22, KCL-MTH-10-10, UMTG-270, UUITP-41-10",
    doi = "10.1007/s11005-011-0529-2",
    journal = "Lett. Math. Phys.",
    volume = "99",
    pages = "3--32",
    year = "2012"
}

@article{Beisert:2005if,%BeisertRoiban_2004_GammaDef
    author = "Beisert, N. and Roiban, R.",
    title = "{Beauty and the twist: The Bethe ansatz for twisted N=4 SYM}",
    eprint = "hep-th/0505187",
    archivePrefix = "arXiv",
    reportNumber = "PUTP-2162",
    doi = "10.1088/1126-6708/2005/08/039",
    journal = "JHEP",
    volume = "08",
    pages = "039",
    year = "2005"
}

@article{DEramo:1971hnd,%FirstUniqueness
    author = "D'Eramo, M. and Parisi, G. and Peliti, L.",
    title = "{THEORETICAL PREDICTIONS FOR CRITICAL EXPONENTS AT THE lambda POINT OF BOSE LIQUIDS}",
    reportNumber = "LNF-71-67",
    doi = "10.1007/BF02774121",
    journal = "Lett. Nuovo Cim.",
    volume = "2",
    number = "17",
    pages = "878--880",
    year = "1971"
}

@article{UniquenessDIKazakov,
  title={Calculation of Feynman diagrams by the “Uniqueness” method},
  author={Kazakov, Dmitri Igorevich},
  url = {\url{https://link.springer.com/article/10.1007/BF01018044}},
  journal={Teoreticheskaya i Matematicheskaya Fizika},
  volume={58},
  number={3},
  pages={343--353},
  year={1984},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}

@article{Chicherin:2012yn,%Chicherin_2013
    author = "Chicherin, D. and Derkachov, S. and Isaev, A. P.",
    title = "{Conformal group: R-matrix and star-triangle relation}",
    eprint = "1206.4150",
    archivePrefix = "arXiv",
    primaryClass = "math-ph",
    doi = "10.1007/JHEP04(2013)020",
    journal = "JHEP",
    volume = "04",
    pages = "020",
    year = "2013"
}

@article{Gurdogan:2015csr,%GurdoganKazakov_2016_Fishnet1
    author = {G\"urdo\u{g}an, \"Omer and Kazakov, Vladimir},
    title = "{New Integrable 4D Quantum Field Theories from Strongly Deformed Planar $\mathcal N = $ 4 Supersymmetric Yang-Mills Theory}",
    eprint = "1512.06704",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevLett.117.201602",
    journal = "Phys. Rev. Lett.",
    volume = "117",
    number = "20",
    pages = "201602",
    year = "2016",
    note = "[Addendum: Phys.Rev.Lett. 117, 259903 (2016)]"
}

@article{Sieg:2016vap,%SiegWilhelm_FishnetDoubleTrace
    author = "Sieg, Christoph and Wilhelm, Matthias",
    title = "{On a CFT limit of planar $\gamma_i$-deformed $\mathcal{N}=4$ SYM theory}",
    eprint = "1602.05817",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "HU-MATHEMATIK-2016-02, \textbackslash{}-HU-EP-16-06, HU-EP-16-06",
    doi = "10.1016/j.physletb.2016.03.004",
    journal = "Phys. Lett. B",
    volume = "756",
    pages = "118--120",
    year = "2016"
}

@article{Fokken:2013aea,%FokkenSiegWilhelm_DoubleTraceGammaDef
    author = "Fokken, Jan and Sieg, Christoph and Wilhelm, Matthias",
    title = "{Non-conformality of ${{\gamma }_{i}}$-deformed N = 4 SYM theory}",
    eprint = "1308.4420",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "HU-MATH-2013-15, HU-EP-13-40",
    doi = "10.1088/1751-8113/47/45/455401",
    journal = "J. Phys. A",
    volume = "47",
    pages = "455401",
    year = "2014"
}

@article{Caetano:2016ydc,%ChiTheoriesAndABJM
    author = {Caetano, Jo\~ao and G\"urdo\u{g}an, \"Omer and Kazakov, Vladimir},
    title = "{Chiral limit of $ \mathcal{N} $ = 4 SYM and ABJM and integrable Feynman graphs}",
    eprint = "1612.05895",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP03(2018)077",
    journal = "JHEP",
    volume = "03",
    pages = "077",
    year = "2018"
}

@article{Gromov:2017cja,%GGKKNS_FishnetIntegrability
    author = "Gromov, Nikolay and Kazakov, Vladimir and Korchemsky, Gregory and Negro, Stefano and Sizov, Grigory",
    title = "{Integrability of Conformal Fishnet Theory}",
    eprint = "1706.04167",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP01(2018)095",
    journal = "JHEP",
    volume = "01",
    pages = "095",
    year = "2018"
}

@article{Chicherin:2017frs,%CKLoebbert_2017_YangianCorrelators
    author = {Chicherin, Dmitry and Kazakov, Vladimir and Loebbert, Florian and M\"uller, Dennis and Zhong, De-liang},
    title = "{Yangian Symmetry for Fishnet Feynman Graphs}",
    eprint = "1708.00007",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MITP-17-049, HU-EP-17-20, LPTENS-17-32",
    doi = "10.1103/PhysRevD.96.121901",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "12",
    pages = "121901",
    year = "2017"
}

@article{Grabner:2017pgm,%GrabnerGKK_FishnetFixedPoints
    author = "Grabner, David and Gromov, Nikolay and Kazakov, Vladimir and Korchemsky, Gregory",
    title = "{Strongly $\gamma$-Deformed $\mathcal{N}=4$ Supersymmetric Yang-Mills Theory as an Integrable Conformal Field Theory}",
    eprint = "1711.04786",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "KCL-MTH-17-04, LPTENS-17-31, IPHT-T17-171, LPTENS--17-31, IPHT--T17-171",
    doi = "10.1103/PhysRevLett.120.111601",
    journal = "Phys. Rev. Lett.",
    volume = "120",
    number = "11",
    pages = "111601",
    year = "2018"
}

@article{Gromov:2018hut,%GromovKK_FishnetExactCorrelationFctns
    author = "Gromov, Nikolay and Kazakov, Vladimir and Korchemsky, Gregory",
    title = "{Exact Correlation Functions in Conformal Fishnet Theory}",
    eprint = "1808.02688",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2019)123",
    journal = "JHEP",
    volume = "08",
    pages = "123",
    year = "2019"
}

@article{Kazakov:2018gcy,%GeneralizedFishnet
    author = "Kazakov, Vladimir and Olivucci, Enrico and Preti, Michelangelo",
    title = "{Generalized fishnets and exact four-point correlators in chiral CFT$_{4}$}",
    eprint = "1901.00011",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP06(2019)078",
    journal = "JHEP",
    volume = "06",
    pages = "078",
    year = "2019"
}

@article{Derkachov:2021rrf,%SpinningRmatrices
    author = "Derkachov, Sergey and Olivucci, Enrico",
    title = "{Conformal quantum mechanics \& the integrable spinning Fishnet}",
    eprint = "2103.01940",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP11(2021)060",
    journal = "JHEP",
    volume = "11",
    pages = "060",
    year = "2021"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Derkachov:2020zvv,%BDdiagramsLong
    author = "Derkachov, Sergey and Olivucci, Enrico",
    title = "{Exactly solvable single-trace four point correlators in $\chi$CFT$_4$}",
    eprint = "2007.15049",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP02(2021)146",
    journal = "JHEP",
    volume = "02",
    pages = "146",
    year = "2021"
}

@article{Kazakov:2022dbd,%FishnetLoom
    author = "Kazakov, Vladimir and Olivucci, Enrico",
    title = "{The loom for general fishnet CFTs}",
    eprint = "2212.09732",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP06(2023)041",
    journal = "JHEP",
    volume = "06",
    pages = "041",
    year = "2023"
}

@article{Preti:2018vog,%PretiGameOfTriangles1
    author = "Preti, Michelangelo",
    title = "{STR: a Mathematica package for the method of uniqueness}",
    eprint = "1811.04935",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1142/S0129183120501466",
    journal = "Int. J. Mod. Phys. C",
    volume = "31",
    number = "10",
    pages = "2050146",
    year = "2020"
}

@article{Preti:2019rcq,%PretiGameOfTriangles2
    author = "Preti, Michelangelo",
    title = "{The Game of Triangles}",
    eprint = "1905.07380",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "NORDITA 2019-047",
    doi = "10.1088/1742-6596/1525/1/012015",
    journal = "J. Phys. Conf. Ser.",
    volume = "1525",
    number = "1",
    pages = "012015",
    year = "2020"
}

@article{Basso:2018agi,%BassoZhong_ContiuumLimitOfFishnetGraphs
    author = "Basso, Benjamin and Zhong, De-liang",
    title = "{Continuum limit of fishnet graphs and AdS sigma model}",
    eprint = "1806.04105",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP01(2019)002",
    journal = "JHEP",
    volume = "01",
    pages = "002",
    year = "2019"
}

@article{Pomoni:2009joh,%PomoniRastelli_doubletrace
    author = "Pomoni, Elli and Rastelli, Leonardo",
    title = "{Large N Field Theory and AdS Tachyons}",
    eprint = "0805.2261",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "YITP-SB-08-20",
    doi = "10.1088/1126-6708/2009/04/020",
    journal = "JHEP",
    volume = "04",
    pages = "020",
    year = "2009"
}

@article{Basso:2017jwq,%BassoDixon_2017_BDdiagrams
    author = "Basso, Benjamin and Dixon, Lance J.",
    title = "{Gluing Ladder Feynman Diagrams into Fishnets}",
    eprint = "1705.03545",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-16967",
    doi = "10.1103/PhysRevLett.119.071601",
    journal = "Phys. Rev. Lett.",
    volume = "119",
    number = "7",
    pages = "071601",
    year = "2017"
}

@article{Gromov:2019aku,%GromovSever_Fishchain1
    author = "Gromov, Nikolay and Sever, Amit",
    title = "{Derivation of the Holographic Dual of a Planar Conformal Field Theory in 4D}",
    eprint = "1903.10508",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-TH-2019-039",
    doi = "10.1103/PhysRevLett.123.081602",
    journal = "Phys. Rev. Lett.",
    volume = "123",
    number = "8",
    pages = "081602",
    year = "2019"
}

@article{Iakhibbaev:2023dye,%IT_ABJMFishchain
    author = "Iakhibbaev, R. M. and Tolkachev, D. M.",
    title = "{Generalising holographic fishchain}",
    eprint = "2308.08914",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2023"
}

